Measurements of prompt charm production cross-sections in $pp$ collisions at $\sqrt{s} = 13\,\mathrm{TeV}$

Production cross-sections of prompt charm mesons are measured with the first data from $pp$ collisions at the LHC at a centre-of-mass energy of $13\,\mathrm{TeV}$. The data sample corresponds to an integrated luminosity of $4.98 \pm 0.19\,\mathrm{pb}^{-1}$ collected by the LHCb experiment. The production cross-sections of $D^{0}$, $D^{+}$, $D_{s}^{+}$, and $D^{*+}$ mesons are measured in bins of charm meson transverse momentum, $p_{\mathrm{T}}$, and rapidity, $y$, and cover the range $0 < p_{\mathrm{T}} < 15\,\mathrm{GeV}/c$ and $2.0 < y < 4.5$. The inclusive cross-sections for the four mesons, including charge conjugation, within the range of $1 < p_{\mathrm{T}} < 8\,\mathrm{GeV}/c$ are found to be \begin{equation} \sigma(pp \to D^{0} X) = 2072 \pm 2 \pm 124\,\mu\mathrm{b}\\ \sigma(pp \to D^{+} X) = 834 \pm 2 \pm \phantom{1}78\,\mu\mathrm{b}\\ \sigma(pp \to D_{s}^{+} X) = 353 \pm 9 \pm \phantom{1}76\,\mu\mathrm{b}\\ \sigma(pp \to D^{*+} X) = 784 \pm 4 \pm \phantom{1}87\,\mu\mathrm{b} \end{equation} where the uncertainties are due to statistical and systematic uncertainties, respectively.

==> lhcb-symbols-def.tex <==
\def\lhcb {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}

\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace}
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pizs   {{\ensuremath{\pion^0\mbox\,\rm{s}}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
  \def\Kbar    {{\kern 0.2em\overline{\kern -0.2em \PK}{}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\rm\scriptscriptstyle S}}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\rm\scriptscriptstyle L}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

  \def\Dbar    {{\kern 0.2em\overline{\kern -0.2em \PD}{}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

\def\B       {{\ensuremath{\PB}}\xspace}
\def\Bbar    {{\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}

\def\chic  {{\ensuremath{\Pchi_{c}}}\xspace}

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresbar    {{\ensuremath{\overline \Xires}}\xspace}
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}}\xspace}
\def\LorLbar    {\kern 0.18em\optbar{\kern -0.18em \PLambda}{}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaresbar {{\ensuremath{\overline \Sigmares}}\xspace}
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\overline \POmega}}\xspace}

\def\Lb      {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar   {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Lc      {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar   {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xib     {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz    {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm    {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar  {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Xic     {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz    {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp    {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar  {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac    {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Omegab    {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

\def\BF         {{\ensuremath{\cal B}}\xspace}
\def\BRvis      {{\ensuremath{\BR_{\rm{vis}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\rm L}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\rm H}}}\xspace}

\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\rm L}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\rm H}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\cal A}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\cal A}^{\rm dir}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\cal A}^{\rm mix}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\cal A}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

\newcommand{\edet}{{\ensuremath{\varepsilon_{\rm det}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\rm rec/det}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\rm sel/rec}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\rm trg/sel}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\rm tot}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\rm comb}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\rm tag}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\rm tag}^{\rm comb}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\rm eff}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\rm eff}^{\rm comb}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\rm tag}^{\rm Pr}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\rm tag}^{\rm LL}}}\xspace}

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}

\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

\newcommand{\bra}[1]{\ensuremath{\langle #1|}}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}}

\newcommand{\unit}[1]{\ensuremath{\rm\,#1}\xspace}

\newcommand{\tev}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}\xspace}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\ma   {\ensuremath{{\rm \,m}^2}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\upmu\rm m}}\xspace}
\def\muma {\ensuremath{{\,\upmu\rm m^2}}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mub{\ensuremath{{\rm \,\upmu b}}\xspace}
\def\nb {\ensuremath{\rm \,nb}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}

\def\sec  {\ensuremath{\rm {\,s}}\xspace}
\def\ms   {\ensuremath{{\rm \,ms}}\xspace}
\def\mus  {\ensuremath{{\,\upmu{\rm s}}}\xspace}
\def\ns   {\ensuremath{{\rm \,ns}}\xspace}
\def\ps   {\ensuremath{{\rm \,ps}}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

\def\mhz  {\ensuremath{{\rm \,MHz}}\xspace}
\def\khz  {\ensuremath{{\rm \,kHz}}\xspace}
\def\hz   {\ensuremath{{\rm \,Hz}}\xspace}

\def\invps{\ensuremath{{\rm \,ps^{-1}}}\xspace}

\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}

\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\rm \,n_{eq}}\xspace}
\def\neqcmcm {\ensuremath{\rm \,n_{eq} / cm^2}\xspace}
\def\kRad {\ensuremath{\rm \,kRad}\xspace}
\def\MRad {\ensuremath{\rm \,MRad}\xspace}
\def\ci {\ensuremath{\rm \,Ci}\xspace}
\def\mci {\ensuremath{\rm \,mCi}\xspace}

\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\ensuremath{\mathrm{\,(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\,(syst)}}\xspace}

\def\order{{\ensuremath{\cal O}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\rm IP}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\rm VS}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\rm vtx}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}

\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_{\rm T}$}\xspace}
\def\et         {\mbox{$E_{\rm T}$}\xspace}
\def\mt         {\mbox{$M_{\rm T}$}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}
\def\rad{\ensuremath{\rm \,rad}\xspace}

\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}

\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{SVN}}\xspace}

\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}

\def\dst        {DST\xspace}

\def\nonn {\ensuremath{\rm {\it{n^+}}\mbox{-}on\mbox{-}{\it{n}}}\xspace}
\def\ponn {\ensuremath{\rm {\it{p^+}}\mbox{-}on\mbox{-}{\it{n}}}\xspace}
\def\nonp {\ensuremath{\rm {\it{n^+}}\mbox{-}on\mbox{-}{\it{p}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

\def\cfourften     {\ensuremath{\rm C_4 F_{10}}\xspace}
\def\cffour        {\ensuremath{\rm CF_4}\xspace}
\def\cotwo         {\ensuremath{\rm CO_2}\xspace} 
\def\csixffouteen  {\ensuremath{\rm C_6 F_{14}}\xspace} 
\def\mgftwo     {\ensuremath{\rm Mg F_2}\xspace} 
\def\siotwo     {\ensuremath{\rm SiO_2}\xspace} 

\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}


==> tables/integrated/integrated_crosssections_ratios.tex <==
\begin{adjustbox}{center}
\begin{tabular}{ccccr}
&& & $R_{13/7}$ \\
\midrule
\Dz   & $0 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $1.64 \pm 0.02  \pm 0.15$\\
\Dp   & $0 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $1.78 \pm 0.03  \pm 0.31$\\
\midrule
\Dz   & $1 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $1.71 \pm 0.02  \pm 0.15$\\
\Dp   & $1 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $1.79 \pm 0.03  \pm 0.30$\\
\Dsp   & $1 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $2.56 \pm 0.19  \pm 0.66$\\
\Dstp   & $1 < \pT < \SI{8}{\GeVc}$ & $2 < \rapidity < 4.5$   & $1.67 \pm 0.05  \pm 0.24$\\
\midrule
\end{tabular}
\end{adjustbox}


==> tables/mode_ratios/Dp_by_D0.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[0,1000]$ & $\phantom{.}\phantom{0}\phantom{0}30\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}21\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}33.5\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}6.9\phantom{0}}_{-\phantom{.}7.1\phantom{0}}$ & $\phantom{0}37.8\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}7.2\phantom{0}}$ & $\phantom{0}26.1\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}30.6\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}2.0}$$\phantom{.}^{+\phantom{.}7.1\phantom{0}}_{-\phantom{.}7.3\phantom{0}}$ \\
$[1000,1500]$ & $\phantom{0}32.9\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}6.9\phantom{0}}$ & $\phantom{0}42.6\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}5.8\phantom{0}}$ & $\phantom{0}41.9\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}5.5\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}39.3\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ & $\phantom{0}39.8\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}4.4\phantom{0}}$ \\
$[1500,2000]$ & $\phantom{0}45.8\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}5.8\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $\phantom{0}39.6\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}41.0\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{0}37.2\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}3.5\phantom{0}}$ & $\phantom{0}42.2\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{0}41.5\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}4.0\phantom{0}}_{-\phantom{.}2.9\phantom{0}}$ & $\phantom{0}39.2\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}3.3\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}39.5\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}3.6\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}38.5\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}40.3\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}3.0\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{0}44.0\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}3.1\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}38.6\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}40.7\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}3.0\phantom{0}}_{-\phantom{.}2.8\phantom{0}}$ & $\phantom{0}37.9\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}40.1\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.9\phantom{0}}_{-\phantom{.}2.8\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{0}42.1\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}41.6\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}41.9\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.7\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}39.7\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}44.7\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}3.2\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ \\
$[3500,4000]$ & $\phantom{0}40.2\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}40.9\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}39.3\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{0}48.1\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ \\
$[4000,5000]$ & $\phantom{0}42.6\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}41.9\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}41.5\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}43.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}45.9\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}5.5\phantom{0}}_{-\phantom{.}5.0\phantom{0}}$ \\
$[5000,6000]$ & $\phantom{0}42.6\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{0}41.2\phantom{.}^{+\phantom{.}0.2}_{-\phantom{.}0.2}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}45.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}44.3\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.7\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}67\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}46.4\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}40.6\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}44.5\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}50.9\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}3.8\phantom{0}}$ & $\phantom{.}\phantom{0}101\phantom{.}^{+\phantom{.}18}_{-\phantom{.}14}$$\phantom{.}^{+\phantom{.}58\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}41\phantom{.}\phantom{0}\phantom{.}}$ \\
$[7000,8000]$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}3.0\phantom{0}}_{-\phantom{.}2.8\phantom{0}}$ & $\phantom{0}41.8\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}44.1\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}56.2\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}6.3\phantom{0}}$ &  \\
$[8000,9000]$ & $\phantom{0}45.4\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}3.3\phantom{0}}_{-\phantom{.}3.5\phantom{0}}$ & $\phantom{0}44.2\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.7\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}45.6\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ & $\phantom{0}45.1\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}7.1\phantom{0}}_{-\phantom{.}6.6\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}39.6\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}41.4\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{0}45.2\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}60\phantom{.}^{+\phantom{.}5}_{-\phantom{.}4}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[10000,11000]$ & $\phantom{0}45.7\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}43.5\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}47.5\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}65\phantom{.}^{+\phantom{.}14}_{-\phantom{.}10}$$\phantom{.}^{+\phantom{.}16\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}15\phantom{.}\phantom{0}\phantom{.}}$ &  \\
$[11000,12000]$ & $\phantom{0}50.7\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}49.4\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ &  &  \\
$[12000,13000]$ & $\phantom{0}50.7\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.9}$$\phantom{.}^{+\phantom{.}3.6\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}45.0\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ &  &  \\
$[13000,14000]$ & $\phantom{0}48.7\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.1}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}41.4\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}53.3\phantom{.}^{+\phantom{.}4.4}_{-\phantom{.}4.0}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}53.3\phantom{.}^{+\phantom{.}3.1}_{-\phantom{.}2.8}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}43.7\phantom{.}^{+\phantom{.}2.3}_{-\phantom{.}2.1}$$\phantom{.}^{+\phantom{.}3.2\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}61\phantom{.}^{+\phantom{.}8}_{-\phantom{.}7}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}7\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ &  &  \\
\end{tabular}


==> tables/mode_ratios/Ds_by_D0.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[1000,1500]$ & $\phantom{0}14.9\phantom{.}^{+\phantom{.}3.7}_{-\phantom{.}3.7}$$\phantom{.}^{+\phantom{.}7.3\phantom{0}}_{-\phantom{.}8.3\phantom{0}}$ & $\phantom{0}12.8\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}15.2\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.5\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}18.2\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}38\phantom{.}^{+\phantom{.}12}_{-\phantom{.}12}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}25\phantom{.}\phantom{0}\phantom{.}}$ \\
$[1500,2000]$ & $\phantom{0}12.5\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}15.9\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}19.2\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}18.7\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}13.1\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{0}19.7\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}18.3\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}17.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}17.6\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.4\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}15.7\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}2.4\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{0}20.5\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.8\phantom{0}}$ & $\phantom{0}19.2\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}21.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}18.4\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}15.1\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{0}19.4\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}20.6\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}20.6\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}17.8\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.6\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}20.3\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ \\
$[3500,4000]$ & $\phantom{0}22.7\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}20.2\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}20.0\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}20.8\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.6\phantom{0}}$ & $\phantom{0}20.5\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ \\
$[4000,5000]$ & $\phantom{0}19.1\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.6\phantom{0}}$ & $\phantom{0}21.1\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.3\phantom{0}}$ & $\phantom{0}18.9\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.4\phantom{0}}_{-\phantom{.}1.3\phantom{0}}$ & $\phantom{0}20.5\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.6\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}20.5\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.1\phantom{0}}_{-\phantom{.}2.9\phantom{0}}$ \\
$[5000,6000]$ & $\phantom{0}19.9\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.6\phantom{0}}$ & $\phantom{0}20.9\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}23.0\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}23.5\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}33.5\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.5}$$\phantom{.}^{+\phantom{.}5.9\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}21.8\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}21.4\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}20.0\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}24.5\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}52\phantom{.}^{+\phantom{.}11}_{-\phantom{.}9}$$\phantom{.}^{+\phantom{.}31\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}22\phantom{.}\phantom{0}\phantom{.}}$ \\
$[7000,8000]$ & $\phantom{0}25.5\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}2.9\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}22.1\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}19.8\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}30.9\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ &  \\
$[8000,9000]$ & $\phantom{0}22.2\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}20.9\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}21.0\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}24.4\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}5.5\phantom{0}}_{-\phantom{.}4.5\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}20.4\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}2.3\phantom{0}}$ & $\phantom{0}17.1\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.3\phantom{0}}$ & $\phantom{0}24.2\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}22.4\phantom{.}^{+\phantom{.}2.8}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}5.7\phantom{0}}_{-\phantom{.}5.3\phantom{0}}$ &  \\
$[10000,11000]$ & $\phantom{0}23.9\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}21.6\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.1\phantom{0}}$ & $\phantom{0}22.1\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}1.0\phantom{0}}$ & $\phantom{0}25.4\phantom{.}^{+\phantom{.}7.2}_{-\phantom{.}5.6}$$\phantom{.}^{+\phantom{.}9.3\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ &  \\
$[11000,12000]$ & $\phantom{0}24.1\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.9}$$\phantom{.}^{+\phantom{.}2.5\phantom{0}}_{-\phantom{.}1.2\phantom{0}}$ & $\phantom{0}19.8\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}0.8\phantom{0}}$ & $\phantom{0}24.0\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}1.9}$$\phantom{.}^{+\phantom{.}2.7\phantom{0}}_{-\phantom{.}1.1\phantom{0}}$ &  &  \\
$[12000,13000]$ & $\phantom{0}27.4\phantom{.}^{+\phantom{.}2.4}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}1.1\phantom{0}}$ & $\phantom{0}16.9\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}1.7\phantom{0}}_{-\phantom{.}0.7\phantom{0}}$ & $\phantom{0}24.9\phantom{.}^{+\phantom{.}2.8}_{-\phantom{.}2.5}$$\phantom{.}^{+\phantom{.}3.6\phantom{0}}_{-\phantom{.}1.3\phantom{0}}$ &  &  \\
$[13000,14000]$ & $\phantom{0}20.0\phantom{.}^{+\phantom{.}2.4}_{-\phantom{.}2.3}$$\phantom{.}^{+\phantom{.}2.8\phantom{0}}_{-\phantom{.}0.4\phantom{0}}$ & $\phantom{0}22.1\phantom{.}^{+\phantom{.}2.1}_{-\phantom{.}2.0}$$\phantom{.}^{+\phantom{.}2.3\phantom{0}}_{-\phantom{.}1.1\phantom{0}}$ & $\phantom{0}26.2\phantom{.}^{+\phantom{.}4.1}_{-\phantom{.}3.8}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}0.7\phantom{0}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}17.9\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}2.5}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ & $\phantom{0}23.4\phantom{.}^{+\phantom{.}4.9}_{-\phantom{.}2.5}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ & $\phantom{0}27.7\phantom{.}^{+\phantom{.}9.5}_{-\phantom{.}5.4}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ &  &  \\
\end{tabular}


==> tables/mode_ratios/Ds_by_Dp.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[1000,1500]$ & $\phantom{.}\phantom{0}\phantom{0}45\phantom{.}^{+\phantom{.}11}_{-\phantom{.}11}$$\phantom{.}^{+\phantom{.}24\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}25\phantom{.}\phantom{0}\phantom{.}}$ & $\phantom{0}30.1\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}36.3\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}6.0\phantom{0}}_{-\phantom{.}5.2\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}46\phantom{.}^{+\phantom{.}5}_{-\phantom{.}5}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}96\phantom{.}^{+\phantom{.}31}_{-\phantom{.}31}$$\phantom{.}^{+\phantom{.}33\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}63\phantom{.}\phantom{0}\phantom{.}}$ \\
$[1500,2000]$ & $\phantom{0}27.3\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}5.7\phantom{0}}_{-\phantom{.}5.0\phantom{0}}$ & $\phantom{0}40.1\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{0}46.9\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ & $\phantom{0}50.3\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}31.1\phantom{.}^{+\phantom{.}3.2}_{-\phantom{.}3.2}$$\phantom{.}^{+\phantom{.}6.9\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{0}47.5\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}7.8\phantom{0}}_{-\phantom{.}6.2\phantom{0}}$ & $\phantom{0}46.6\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}44.2\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.4\phantom{0}}_{-\phantom{.}3.4\phantom{0}}$ & $\phantom{0}45.8\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}39.1\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}4.9\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{0}46.7\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}6.0\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}49.7\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}52.6\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}48.6\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}4.7\phantom{0}}_{-\phantom{.}3.8\phantom{0}}$ & $\phantom{0}37.7\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}4.9\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{0}46.0\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}5.3\phantom{0}}_{-\phantom{.}4.5\phantom{0}}$ & $\phantom{0}49.5\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}4.0\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}49.3\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}3.4\phantom{0}}$ & $\phantom{0}45.3\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}5.8\phantom{0}}_{-\phantom{.}4.7\phantom{0}}$ \\
$[3500,4000]$ & $\phantom{0}56.4\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $\phantom{0}48.1\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}3.3\phantom{0}}$ & $\phantom{0}48.9\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.7\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ & $\phantom{0}52.8\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.9\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{0}42.6\phantom{.}^{+\phantom{.}2.3}_{-\phantom{.}2.3}$$\phantom{.}^{+\phantom{.}5.0\phantom{0}}_{-\phantom{.}4.7\phantom{0}}$ \\
$[4000,5000]$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}50.2\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ & $\phantom{0}45.5\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}3.5\phantom{0}}_{-\phantom{.}3.3\phantom{0}}$ & $\phantom{0}47.2\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ & $\phantom{0}44.7\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}2.0}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ \\
$[5000,6000]$ & $\phantom{0}46.8\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ & $\phantom{0}50.7\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}3.5\phantom{0}}$ & $\phantom{0}50.6\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}53.1\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}4.9\phantom{0}}_{-\phantom{.}4.5\phantom{0}}$ & $\phantom{0}50.0\phantom{.}^{+\phantom{.}3.3}_{-\phantom{.}3.3}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}6.0\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}47.1\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ & $\phantom{0}52.6\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.7\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ & $\phantom{0}45.0\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}3.4\phantom{0}}$ & $\phantom{0}48.1\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}5.1\phantom{0}}_{-\phantom{.}4.6\phantom{0}}$ & $\phantom{0}51.1\phantom{.}^{+\phantom{.}6.1}_{-\phantom{.}6.1}$$\phantom{.}^{+\phantom{.}9.2\phantom{0}}_{-\phantom{.}8.2\phantom{0}}$ \\
$[7000,8000]$ & $\phantom{0}56.7\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}2.0}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}5.9\phantom{0}}$ & $\phantom{0}52.9\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}5.1\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{0}44.8\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}3.7\phantom{0}}$ & $\phantom{0}55.0\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $\phantom{0}26.0\phantom{.}^{+\phantom{.}7.0}_{-\phantom{.}6.8}$$\phantom{.}^{+\phantom{.}8.7\phantom{0}}_{-\phantom{.}6.6\phantom{0}}$ \\
$[8000,9000]$ & $\phantom{0}49.0\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}2.1}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}47.4\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}5.2\phantom{0}}_{-\phantom{.}4.1\phantom{0}}$ & $\phantom{0}46.1\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.7}$$\phantom{.}^{+\phantom{.}5.0\phantom{0}}_{-\phantom{.}4.1\phantom{0}}$ & $\phantom{0}54.1\phantom{.}^{+\phantom{.}3.7}_{-\phantom{.}3.6}$$\phantom{.}^{+\phantom{.}7.8\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}51.5\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.8\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}41.2\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}4.6\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ & $\phantom{0}53.5\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.6\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{0}37.5\phantom{.}^{+\phantom{.}3.7}_{-\phantom{.}3.7}$$\phantom{.}^{+\phantom{.}5.4\phantom{0}}_{-\phantom{.}4.2\phantom{0}}$ &  \\
$[10000,11000]$ & $\phantom{0}52.3\phantom{.}^{+\phantom{.}3.2}_{-\phantom{.}3.2}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ & $\phantom{0}49.7\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.7}$$\phantom{.}^{+\phantom{.}4.2\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}46.5\phantom{.}^{+\phantom{.}3.0}_{-\phantom{.}3.0}$$\phantom{.}^{+\phantom{.}5.6\phantom{0}}_{-\phantom{.}2.3\phantom{0}}$ & $\phantom{0}38.7\phantom{.}^{+\phantom{.}7.0}_{-\phantom{.}6.8}$$\phantom{.}^{+\phantom{.}5.9\phantom{0}}_{-\phantom{.}3.3\phantom{0}}$ &  \\
$[11000,12000]$ & $\phantom{0}47.5\phantom{.}^{+\phantom{.}3.6}_{-\phantom{.}3.6}$$\phantom{.}^{+\phantom{.}4.7\phantom{0}}_{-\phantom{.}2.3\phantom{0}}$ & $\phantom{0}47.1\phantom{.}^{+\phantom{.}3.1}_{-\phantom{.}3.0}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}48.7\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}3.8}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0.}36\phantom{.}^{+\phantom{.}14}_{-\phantom{.}10}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ &  \\
$[12000,13000]$ & $\phantom{0}54.2\phantom{.}^{+\phantom{.}4.8}_{-\phantom{.}4.7}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}1.5\phantom{0}}$ & $\phantom{0}40.3\phantom{.}^{+\phantom{.}3.5}_{-\phantom{.}3.5}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}55.3\phantom{.}^{+\phantom{.}5.6}_{-\phantom{.}5.5}$$\phantom{.}^{+\phantom{.}5.6\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}33\phantom{.}^{+\phantom{.}11}_{-\phantom{.}11}$$\phantom{.}^{+\phantom{.}7\phantom{.}\phantom{0}\phantom{0}\phantom{.}}_{-\phantom{.}4\phantom{.}\phantom{0}\phantom{0}\phantom{.}}$ &  \\
$[13000,14000]$ & $\phantom{0}41.2\phantom{.}^{+\phantom{.}4.8}_{-\phantom{.}4.8}$$\phantom{.}^{+\phantom{.}5.2\phantom{0}}_{-\phantom{.}0.9\phantom{0}}$ & $\phantom{0}53.4\phantom{.}^{+\phantom{.}4.8}_{-\phantom{.}4.7}$$\phantom{.}^{+\phantom{.}5.6\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}49.1\phantom{.}^{+\phantom{.}6.9}_{-\phantom{.}6.8}$$\phantom{.}^{+\phantom{.}7.6\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}33.6\phantom{.}^{+\phantom{.}5.0}_{-\phantom{.}4.8}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}0.6\phantom{0}}$ & $\phantom{0.}53\phantom{.}^{+\phantom{.}10}_{-\phantom{.}6}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ & $\phantom{0}45.1\phantom{.}^{+\phantom{.}8.6}_{-\phantom{.}8.4}$$\phantom{.}^{+\phantom{.}9.4\phantom{0}}_{-\phantom{.}0.5\phantom{0}}$ &  &  \\
\end{tabular}


==> tables/mode_ratios/Ds_by_Dst.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[1000,1500]$ &  & $\phantom{.}\phantom{0}\phantom{0}42\phantom{.}^{+\phantom{.}4}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}13\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}41.6\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.4\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}58\phantom{.}^{+\phantom{.}6}_{-\phantom{.}6}$$\phantom{.}^{+\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}93\phantom{.}^{+\phantom{.}30}_{-\phantom{.}30}$$\phantom{.}^{+\phantom{.}34\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}62\phantom{.}\phantom{0}\phantom{.}}$ \\
$[1500,2000]$ &  & $\phantom{0}40.9\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}7.1\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $\phantom{0}47.5\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}5.3\phantom{0}}_{-\phantom{.}5.5\phantom{0}}$ & $\phantom{0}48.8\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}9.0\phantom{0}}_{-\phantom{.}8.6\phantom{0}}$ & $\phantom{0}33.6\phantom{.}^{+\phantom{.}3.6}_{-\phantom{.}3.5}$$\phantom{.}^{+\phantom{.}9.6\phantom{0}}_{-\phantom{.}8.0\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{.}\phantom{0}\phantom{0}65\phantom{.}^{+\phantom{.}7}_{-\phantom{.}6}$$\phantom{.}^{+\phantom{.}26\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}44.3\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}4.6\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}39.8\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}5.2\phantom{0}}_{-\phantom{.}4.8\phantom{0}}$ & $\phantom{0}43.3\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}7.9\phantom{0}}_{-\phantom{.}7.4\phantom{0}}$ & $\phantom{0}36.0\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}8.8\phantom{0}}_{-\phantom{.}6.9\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{0}49.6\phantom{.}^{+\phantom{.}2.3}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}9.9\phantom{0}}_{-\phantom{.}7.6\phantom{0}}$ & $\phantom{0}45.7\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}47.1\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}6.0\phantom{0}}$ & $\phantom{0}43.2\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}8.8\phantom{0}}_{-\phantom{.}7.4\phantom{0}}$ & $\phantom{0}35.1\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}5.5\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{0}44.2\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $\phantom{0}48.3\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.0\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}46.5\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}5.9\phantom{0}}$ & $\phantom{0}42.4\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}9.0\phantom{0}}_{-\phantom{.}7.4\phantom{0}}$ & $\phantom{0}42.2\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}8.5\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ \\
$[3500,4000]$ & $\phantom{0}53.0\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.7}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}45.0\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.3\phantom{0}}$ & $\phantom{0}41.2\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}6.9\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $\phantom{0}45.9\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}9.6\phantom{0}}_{-\phantom{.}8.0\phantom{0}}$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}2.7}_{-\phantom{.}2.7}$$\phantom{.}^{+\phantom{.}6.9\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ \\
$[4000,5000]$ & $\phantom{0}42.6\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}3.8\phantom{0}}_{-\phantom{.}3.8\phantom{0}}$ & $\phantom{0}48.0\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}3.9\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{0}40.7\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}6.9\phantom{0}}_{-\phantom{.}4.8\phantom{0}}$ & $\phantom{0}44.4\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}8.5\phantom{0}}_{-\phantom{.}7.4\phantom{0}}$ & $\phantom{0}44.2\phantom{.}^{+\phantom{.}2.3}_{-\phantom{.}2.2}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}6.1\phantom{0}}$ \\
$[5000,6000]$ & $\phantom{0}43.4\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}3.8\phantom{0}}$ & $\phantom{0}47.3\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ & $\phantom{0}46.5\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}7.7\phantom{0}}_{-\phantom{.}5.9\phantom{0}}$ & $\phantom{0}47.0\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}62\phantom{.}^{+\phantom{.}5}_{-\phantom{.}5}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}50.2\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}5.1\phantom{0}}_{-\phantom{.}4.8\phantom{0}}$ & $\phantom{0}46.1\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}3.3\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}6.6\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $\phantom{0}51.0\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}5.9\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}80\phantom{.}^{+\phantom{.}18}_{-\phantom{.}14}$$\phantom{.}^{+\phantom{.}24\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}16\phantom{.}\phantom{0}\phantom{.}}$ \\
$[7000,8000]$ & $\phantom{0}47.8\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}5.8\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $\phantom{0}47.0\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}38.6\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}5.7\phantom{0}}_{-\phantom{.}4.5\phantom{0}}$ & $\phantom{0}54.4\phantom{.}^{+\phantom{.}2.9}_{-\phantom{.}2.9}$$\phantom{.}^{+\phantom{.}7.7\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ &  \\
$[8000,9000]$ & $\phantom{0}47.2\phantom{.}^{+\phantom{.}2.1}_{-\phantom{.}2.1}$$\phantom{.}^{+\phantom{.}6.4\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}41.1\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}3.6\phantom{0}}$ & $\phantom{0}41.5\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}4.7\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}55\phantom{.}^{+\phantom{.}4}_{-\phantom{.}4}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}9\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}52.4\phantom{.}^{+\phantom{.}2.9}_{-\phantom{.}2.9}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}6.0\phantom{0}}$ & $\phantom{0}35.8\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}4.4\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}48.6\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.5}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}4.5\phantom{0}}$ & $\phantom{0}45.2\phantom{.}^{+\phantom{.}6.1}_{-\phantom{.}5.4}$$\phantom{.}^{+\phantom{.}9.0\phantom{0}}_{-\phantom{.}6.6\phantom{0}}$ &  \\
$[10000,11000]$ & $\phantom{0}48.0\phantom{.}^{+\phantom{.}3.3}_{-\phantom{.}3.2}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}43.0\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}1.9\phantom{0}}$ & $\phantom{0}41.8\phantom{.}^{+\phantom{.}2.9}_{-\phantom{.}2.9}$$\phantom{.}^{+\phantom{.}4.9\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}46\phantom{.}^{+\phantom{.}13}_{-\phantom{.}10}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}6\phantom{.}\phantom{0}\phantom{0}\phantom{.}}$ &  \\
$[11000,12000]$ & $\phantom{0}45.8\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}3.7}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}43.6\phantom{.}^{+\phantom{.}3.0}_{-\phantom{.}3.0}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}1.3\phantom{0}}$ & $\phantom{0}50.1\phantom{.}^{+\phantom{.}4.5}_{-\phantom{.}4.3}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ &  &  \\
$[12000,13000]$ & $\phantom{0}55.2\phantom{.}^{+\phantom{.}5.3}_{-\phantom{.}4.9}$$\phantom{.}^{+\phantom{.}7.7\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}34.1\phantom{.}^{+\phantom{.}3.2}_{-\phantom{.}3.1}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}0.8\phantom{0}}$ & $\phantom{0}48.9\phantom{.}^{+\phantom{.}5.7}_{-\phantom{.}5.3}$$\phantom{.}^{+\phantom{.}5.8\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ &  &  \\
$[13000,14000]$ & $\phantom{0}36.3\phantom{.}^{+\phantom{.}7.0}_{-\phantom{.}4.5}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ & $\phantom{0}51.4\phantom{.}^{+\phantom{.}5.1}_{-\phantom{.}4.9}$$\phantom{.}^{+\phantom{.}6.8\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}41.4\phantom{.}^{+\phantom{.}7.0}_{-\phantom{.}6.3}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}0.9\phantom{0}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}36.4\phantom{.}^{+\phantom{.}5.9}_{-\phantom{.}5.5}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}1.4\phantom{0}}$ & $\phantom{0}43.6\phantom{.}^{+\phantom{.}9.6}_{-\phantom{.}4.7}$$^{+\phantom{.}0.0}_{-\phantom{.}0.0}$ & $\phantom{.}\phantom{0}\phantom{0}61\phantom{.}^{+\phantom{.}15}_{-\phantom{.}13}$$\phantom{.}^{+\phantom{.}23\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}6\phantom{.}\phantom{0}\phantom{0}\phantom{.}}$ &  &  \\
\end{tabular}


==> tables/mode_ratios/Dst_by_D0.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[0,1000]$ &  &  &  &  & $\phantom{0}17.5\phantom{.}^{+\phantom{.}2.4}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}5.2\phantom{0}}$ \\
$[1000,1500]$ &  & $\phantom{0}30.4\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}5.9\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $\phantom{0}36.6\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}6.0\phantom{0}}$ & $\phantom{0}31.3\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}5.3\phantom{0}}$ & $\phantom{0}41.0\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}9.9\phantom{0}}_{-\phantom{.}7.8\phantom{0}}$ \\
$[1500,2000]$ &  & $\phantom{0}38.9\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}4.1\phantom{0}}_{-\phantom{.}4.7\phantom{0}}$ & $\phantom{0}40.5\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}8.0\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ & $\phantom{0}38.3\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}7.5\phantom{0}}_{-\phantom{.}6.6\phantom{0}}$ & $\phantom{0}39.0\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{0}30.3\phantom{.}^{+\phantom{.}2.7}_{-\phantom{.}2.8}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ & $\phantom{0}41.3\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}3.1\phantom{0}}_{-\phantom{.}3.0\phantom{0}}$ & $\phantom{0}43.8\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ & $\phantom{0}40.7\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}7.9\phantom{0}}_{-\phantom{.}6.7\phantom{0}}$ & $\phantom{0}43.7\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}8.5\phantom{0}}_{-\phantom{.}7.0\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{0}41.5\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}4.6\phantom{0}}_{-\phantom{.}5.2\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}45.5\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}7.9\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ & $\phantom{0}42.7\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}8.6\phantom{0}}_{-\phantom{.}7.0\phantom{0}}$ & $\phantom{0}43.1\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}6.0\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{0}43.8\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.0\phantom{0}}_{-\phantom{.}4.0\phantom{0}}$ & $\phantom{0}42.7\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}44.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ & $\phantom{0}42.0\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}8.5\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ & $\phantom{0}48.0\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ \\
$[3500,4000]$ & $\phantom{0}42.8\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.4\phantom{0}}_{-\phantom{.}3.2\phantom{0}}$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}2.1\phantom{0}}_{-\phantom{.}1.8\phantom{0}}$ & $\phantom{0}48.6\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}7.0\phantom{0}}_{-\phantom{.}6.9\phantom{0}}$ & $\phantom{0}45.3\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}9.1\phantom{0}}_{-\phantom{.}7.3\phantom{0}}$ & $\phantom{0}45.6\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}5.6\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ \\
$[4000,5000]$ & $\phantom{0}44.9\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}43.8\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.6\phantom{0}}$ & $\phantom{0}46.4\phantom{.}^{+\phantom{.}0.3}_{-\phantom{.}0.3}$$\phantom{.}^{+\phantom{.}6.0\phantom{0}}_{-\phantom{.}6.3\phantom{0}}$ & $\phantom{0}46.2\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}8.4\phantom{0}}_{-\phantom{.}6.9\phantom{0}}$ & $\phantom{0}46.5\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ \\
$[5000,6000]$ & $\phantom{0}45.8\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}3.0\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}44.1\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}1.8\phantom{0}}_{-\phantom{.}1.7\phantom{0}}$ & $\phantom{0}49.4\phantom{.}^{+\phantom{.}0.4}_{-\phantom{.}0.4}$$\phantom{.}^{+\phantom{.}6.4\phantom{0}}_{-\phantom{.}6.1\phantom{0}}$ & $\phantom{0}50.1\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}7.4\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ & $\phantom{0}54.0\phantom{.}^{+\phantom{.}3.6}_{-\phantom{.}3.4}$$\phantom{.}^{+\phantom{.}7.2\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}43.5\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}3.0\phantom{0}}_{-\phantom{.}2.4\phantom{0}}$ & $\phantom{0}46.4\phantom{.}^{+\phantom{.}0.5}_{-\phantom{.}0.5}$$\phantom{.}^{+\phantom{.}2.0\phantom{0}}_{-\phantom{.}2.0\phantom{0}}$ & $\phantom{0}47.7\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.6}$$\phantom{.}^{+\phantom{.}5.5\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ & $\phantom{0}48.0\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}5.4\phantom{0}}_{-\phantom{.}4.9\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}65\phantom{.}^{+\phantom{.}17}_{-\phantom{.}13}$$\phantom{.}^{+\phantom{.}38\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}28\phantom{.}\phantom{0}\phantom{.}}$ \\
$[7000,8000]$ & $\phantom{0}53.4\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.7\phantom{0}}$ & $\phantom{0}47.1\phantom{.}^{+\phantom{.}0.6}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}2.9\phantom{0}}_{-\phantom{.}2.3\phantom{0}}$ & $\phantom{0}51.2\phantom{.}^{+\phantom{.}0.8}_{-\phantom{.}0.8}$$\phantom{.}^{+\phantom{.}5.6\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ & $\phantom{0}56.8\phantom{.}^{+\phantom{.}1.9}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}7.4\phantom{0}}_{-\phantom{.}6.8\phantom{0}}$ &  \\
$[8000,9000]$ & $\phantom{0}47.1\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.8\phantom{0}}$ & $\phantom{0}51.0\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}3.2\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}50.7\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.1}$$\phantom{.}^{+\phantom{.}4.8\phantom{0}}_{-\phantom{.}5.3\phantom{0}}$ & $\phantom{0}44.6\phantom{.}^{+\phantom{.}2.8}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}6.6\phantom{0}}_{-\phantom{.}5.6\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}39.0\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}2.6\phantom{0}}_{-\phantom{.}2.7\phantom{0}}$ & $\phantom{0}47.6\phantom{.}^{+\phantom{.}1.1}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}1.9\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}49.8\phantom{.}^{+\phantom{.}1.4}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}3.3\phantom{0}}_{-\phantom{.}3.9\phantom{0}}$ & $\phantom{0}49.4\phantom{.}^{+\phantom{.}5.9}_{-\phantom{.}5.3}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}9.0\phantom{0}}$ &  \\
$[10000,11000]$ & $\phantom{0}49.7\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.8}$$\phantom{.}^{+\phantom{.}2.2\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}50.1\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.4}$$\phantom{.}^{+\phantom{.}1.2\phantom{0}}_{-\phantom{.}2.1\phantom{0}}$ & $\phantom{0}52.7\phantom{.}^{+\phantom{.}2.1}_{-\phantom{.}2.0}$$\phantom{.}^{+\phantom{.}3.4\phantom{0}}_{-\phantom{.}3.1\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}55\phantom{.}^{+\phantom{.}16}_{-\phantom{.}12}$$\phantom{.}^{+\phantom{.}22\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}18\phantom{.}\phantom{0}\phantom{.}}$ &  \\
$[11000,12000]$ & $\phantom{0}52.6\phantom{.}^{+\phantom{.}2.3}_{-\phantom{.}2.3}$$\phantom{.}^{+\phantom{.}2.9\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}45.4\phantom{.}^{+\phantom{.}1.6}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}1.2\phantom{0}}_{-\phantom{.}2.2\phantom{0}}$ & $\phantom{0}48.0\phantom{.}^{+\phantom{.}2.7}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}2.9\phantom{0}}_{-\phantom{.}2.9\phantom{0}}$ &  &  \\
$[12000,13000]$ & $\phantom{0}49.8\phantom{.}^{+\phantom{.}2.7}_{-\phantom{.}2.7}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.7\phantom{0}}$ & $\phantom{0}49.5\phantom{.}^{+\phantom{.}2.2}_{-\phantom{.}2.1}$$\phantom{.}^{+\phantom{.}1.4\phantom{0}}_{-\phantom{.}2.6\phantom{0}}$ & $\phantom{0}50.9\phantom{.}^{+\phantom{.}4.0}_{-\phantom{.}3.7}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}2.3\phantom{0}}$ &  &  \\
$[13000,14000]$ & $\phantom{0}55.4\phantom{.}^{+\phantom{.}3.5}_{-\phantom{.}3.4}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}3.5\phantom{0}}$ & $\phantom{0}43.0\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.5}$$\phantom{.}^{+\phantom{.}1.4\phantom{0}}_{-\phantom{.}2.9\phantom{0}}$ & $\phantom{0}63.3\phantom{.}^{+\phantom{.}7.2}_{-\phantom{.}6.6}$$\phantom{.}^{+\phantom{.}7.3\phantom{0}}_{-\phantom{.}4.4\phantom{0}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}49.2\phantom{.}^{+\phantom{.}4.2}_{-\phantom{.}3.9}$$\phantom{.}^{+\phantom{.}4.0\phantom{0}}_{-\phantom{.}2.5\phantom{0}}$ & $\phantom{0}53.6\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}3.6}$$\phantom{.}^{+\phantom{.}3.3\phantom{0}}_{-\phantom{.}3.7\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}45\phantom{.}^{+\phantom{.}9}_{-\phantom{.}8}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}9\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ &  &  \\
\end{tabular}


==> tables/mode_ratios/Dst_by_Dp.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccc}
&\multicolumn{5}{c}{$\text{$y$}$}\\
$\text{$p_{\text{T}}$ [\text{MeV}/c]}$ & $[2,2.5]$ & $[2.5,3]$ & $[3,3.5]$ & $[3.5,4]$ & $[4,4.5]$ \\
\midrule
$[0,1000]$ &  &  &  &  & $\phantom{.}\phantom{0}\phantom{0}57\phantom{.}^{+\phantom{.}9}_{-\phantom{.}9}$$\phantom{.}^{+\phantom{.}27\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}17\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[1000,1500]$ &  & $\phantom{.}\phantom{0}\phantom{0}71\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}87.4\phantom{.}^{+\phantom{.}1.3}_{-\phantom{.}1.3}$$\phantom{.}^{+\phantom{.}9.2\phantom{0}}_{-\phantom{.}6.2\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}80\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}8\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}103\phantom{.}^{+\phantom{.}4}_{-\phantom{.}4}$$\phantom{.}^{+\phantom{.}23\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[1500,2000]$ &  & $\phantom{0}98.2\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.7}$$\phantom{.}^{+\phantom{.}7.5\phantom{0}}_{-\phantom{.}9.6\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}99\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}8\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}103\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}92\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[2000,2500]$ & $\phantom{.}\phantom{0}\phantom{0}73\phantom{.}^{+\phantom{.}7}_{-\phantom{.}7}$$\phantom{.}^{+\phantom{.}17\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}17\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $105.4\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}6.3\phantom{0}}_{-\phantom{.}6.3\phantom{0}}$ & $\phantom{.}\phantom{0}111\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}106\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}109\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}17\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[2500,3000]$ & $\phantom{.}\phantom{0}\phantom{0}94\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $108.6\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}1.0}$$\phantom{.}^{+\phantom{.}5.4\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $\phantom{.}\phantom{0}112\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}113\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}18\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}107\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[3000,3500]$ & $\phantom{.}\phantom{0}104\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $102.6\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}5.1\phantom{0}}_{-\phantom{.}4.6\phantom{0}}$ & $\phantom{.}\phantom{0}106\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}106\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}17\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}13\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}107\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[3500,4000]$ & $106.4\phantom{.}^{+\phantom{.}2.4}_{-\phantom{.}2.3}$$\phantom{.}^{+\phantom{.}9.2\phantom{0}}_{-\phantom{.}8.0\phantom{0}}$ & $106.9\phantom{.}^{+\phantom{.}1.0}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}5.7\phantom{0}}_{-\phantom{.}4.4\phantom{0}}$ & $\phantom{.}\phantom{0}119\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}115\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}19\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}94.9\phantom{.}^{+\phantom{.}2.6}_{-\phantom{.}2.6}$$\phantom{.}^{+\phantom{.}8.2\phantom{0}}_{-\phantom{.}8.0\phantom{0}}$ \\
$[4000,5000]$ & $105.3\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ & $104.5\phantom{.}^{+\phantom{.}0.7}_{-\phantom{.}0.7}$$\phantom{.}^{+\phantom{.}4.7\phantom{0}}_{-\phantom{.}4.3\phantom{0}}$ & $\phantom{.}\phantom{0}112\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}13\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}106\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}16\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}101\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}9\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[5000,6000]$ & $107.7\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.6}$$\phantom{.}^{+\phantom{.}6.6\phantom{0}}_{-\phantom{.}6.1\phantom{0}}$ & $107.0\phantom{.}^{+\phantom{.}0.9}_{-\phantom{.}0.9}$$\phantom{.}^{+\phantom{.}4.6\phantom{0}}_{-\phantom{.}4.7\phantom{0}}$ & $\phantom{.}\phantom{0}109\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}113\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}13\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}13\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}81\phantom{.}^{+\phantom{.}4}_{-\phantom{.}4}$$\phantom{.}^{+\phantom{.}15\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ \\
$[6000,7000]$ & $\phantom{0}93.8\phantom{.}^{+\phantom{.}1.7}_{-\phantom{.}1.7}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $114.3\phantom{.}^{+\phantom{.}1.2}_{-\phantom{.}1.2}$$\phantom{.}^{+\phantom{.}5.3\phantom{0}}_{-\phantom{.}5.7\phantom{0}}$ & $\phantom{.}\phantom{0}107\phantom{.}^{+\phantom{.}1}_{-\phantom{.}1}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{0}94.3\phantom{.}^{+\phantom{.}1.8}_{-\phantom{.}1.9}$$\phantom{.}^{+\phantom{.}8.0\phantom{0}}_{-\phantom{.}7.8\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}64\phantom{.}^{+\phantom{.}11}_{-\phantom{.}10}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}12\phantom{.}\phantom{0}\phantom{.}}$ \\
$[7000,8000]$ & $118.8\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}8.5\phantom{0}}_{-\phantom{.}8.6\phantom{0}}$ & $112.6\phantom{.}^{+\phantom{.}1.5}_{-\phantom{.}1.5}$$\phantom{.}^{+\phantom{.}6.7\phantom{0}}_{-\phantom{.}6.4\phantom{0}}$ & $\phantom{.}\phantom{0}116\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}101\phantom{.}^{+\phantom{.}3}_{-\phantom{.}3}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}9\phantom{.}\phantom{0}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[8000,9000]$ & $103.8\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.5}$$\phantom{.}^{+\phantom{.}8.9\phantom{0}}_{-\phantom{.}7.9\phantom{0}}$ & $115.3\phantom{.}^{+\phantom{.}2.0}_{-\phantom{.}1.9}$$\phantom{.}^{+\phantom{.}7.5\phantom{0}}_{-\phantom{.}6.7\phantom{0}}$ & $\phantom{.}\phantom{0}111\phantom{.}^{+\phantom{.}2}_{-\phantom{.}2}$$\phantom{.}^{+\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}99\phantom{.}^{+\phantom{.}5}_{-\phantom{.}5}$$\phantom{.}^{+\phantom{.}14\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}11\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[9000,10000]$ & $\phantom{0}98.2\phantom{.}^{+\phantom{.}3.1}_{-\phantom{.}3.0}$$\phantom{.}^{+\phantom{.}8.4\phantom{0}}_{-\phantom{.}7.3\phantom{0}}$ & $114.9\phantom{.}^{+\phantom{.}2.5}_{-\phantom{.}2.4}$$\phantom{.}^{+\phantom{.}6.5\phantom{0}}_{-\phantom{.}7.2\phantom{0}}$ & $110.2\phantom{.}^{+\phantom{.}2.9}_{-\phantom{.}2.8}$$\phantom{.}^{+\phantom{.}8.4\phantom{0}}_{-\phantom{.}7.8\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}83\phantom{.}^{+\phantom{.}7}_{-\phantom{.}7}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[10000,11000]$ & $109.0\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}3.8}$$\phantom{.}^{+\phantom{.}5.2\phantom{0}}_{-\phantom{.}4.6\phantom{0}}$ & $115.4\phantom{.}^{+\phantom{.}3.2}_{-\phantom{.}3.1}$$\phantom{.}^{+\phantom{.}3.7\phantom{0}}_{-\phantom{.}5.4\phantom{0}}$ & $111.1\phantom{.}^{+\phantom{.}3.9}_{-\phantom{.}3.8}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}3.7\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}84\phantom{.}^{+\phantom{.}15}_{-\phantom{.}15}$$\phantom{.}^{+\phantom{.}18\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}16\phantom{.}\phantom{0}\phantom{.}}$ &  \\
$[11000,12000]$ & $103.6\phantom{.}^{+\phantom{.}4.5}_{-\phantom{.}4.4}$$\phantom{.}^{+\phantom{.}5.5\phantom{0}}_{-\phantom{.}5.1\phantom{0}}$ & $108.1\phantom{.}^{+\phantom{.}3.7}_{-\phantom{.}3.7}$$\phantom{.}^{+\phantom{.}3.6\phantom{0}}_{-\phantom{.}5.8\phantom{0}}$ & $\phantom{0}97.2\phantom{.}^{+\phantom{.}4.8}_{-\phantom{.}4.8}$$\phantom{.}^{+\phantom{.}4.5\phantom{0}}_{-\phantom{.}8.0\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}66\phantom{.}^{+\phantom{.}9}_{-\phantom{.}9}$$\phantom{.}^{+\phantom{.}33\phantom{.}\phantom{0}\phantom{.}\phantom{0}}_{-\phantom{.}31\phantom{.}\phantom{0}\phantom{.}\phantom{0}}$ &  \\
$[12000,13000]$ & $\phantom{0}98.2\phantom{.}^{+\phantom{.}5.1}_{-\phantom{.}5.0}$$\phantom{.}^{+\phantom{.}5.2\phantom{0}}_{-\phantom{.}5.9\phantom{0}}$ & $118.0\phantom{.}^{+\phantom{.}4.9}_{-\phantom{.}4.7}$$\phantom{.}^{+\phantom{.}4.3\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ & $113.1\phantom{.}^{+\phantom{.}7.6}_{-\phantom{.}7.5}$$\phantom{.}^{+\phantom{.}5.9\phantom{0}}_{-\phantom{.}6.5\phantom{0}}$ &  &  \\
$[13000,14000]$ & $113.6\phantom{.}^{+\phantom{.}6.9}_{-\phantom{.}6.7}$$\phantom{.}^{+\phantom{.}6.2\phantom{0}}_{-\phantom{.}7.8\phantom{0}}$ & $103.9\phantom{.}^{+\phantom{.}5.8}_{-\phantom{.}5.6}$$\phantom{.}^{+\phantom{.}3.6\phantom{0}}_{-\phantom{.}7.3\phantom{0}}$ & $\phantom{.}\phantom{0}119\phantom{.}^{+\phantom{.}11}_{-\phantom{.}10}$$\phantom{.}^{+\phantom{.}10\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}10\phantom{.}\phantom{0}\phantom{.}}$ &  &  \\
$[14000,15000]$ & $\phantom{0}92.3\phantom{.}^{+\phantom{.}7.3}_{-\phantom{.}7.1}$$\phantom{.}^{+\phantom{.}7.7\phantom{0}}_{-\phantom{.}7.9\phantom{0}}$ & $122.7\phantom{.}^{+\phantom{.}8.0}_{-\phantom{.}7.6}$$\phantom{.}^{+\phantom{.}5.1\phantom{0}}_{-\phantom{.}9.5\phantom{0}}$ & $\phantom{.}\phantom{0}\phantom{0}74\phantom{.}^{+\phantom{.}11}_{-\phantom{.}11}$$\phantom{.}^{+\phantom{.}12\phantom{.}\phantom{0}\phantom{.}}_{-\phantom{.}13\phantom{.}\phantom{0}\phantom{.}}$ &  &  \\
\end{tabular}

